An Ensemble Noise-Robust K-fold Cross-Validation Selection Method for Noisy Labels

We consider the problem of training robust and accurate deep neural networks (DNNs) when subject to various proportions of noisy labels. Large-scale datasets tend to contain mislabeled samples that can be memorized by DNNs, impeding the performance. With appropriate handling, this degradation can be alleviated. There are two problems to consider: how to distinguish clean samples and how to deal with noisy samples. In this paper, we present Ensemble Noise-robust K-fold Cross-Validation Selection (E-NKCVS) to effectively select clean samples from noisy data, solving the first problem. For the second problem, we create a new pseudo label for any sample determined to have an uncertain or likely corrupt label. E-NKCVS obtains multiple predicted labels for each sample and the entropy of these labels is used to tune the weight given to the pseudo label and the given label. Theoretical analysis and extensive verification of the algorithms in the noisy label setting are provided. We evaluate our approach on various image and text classification tasks where the labels have been manually corrupted with different noise ratios. Additionally, two large real-world noisy datasets are also used, Clothing-1M and WebVision. E-NKCVS is empirically shown to be highly tolerant to considerable proportions of label noise and has a consistent improvement over state-of-the-art methods. Especially on more difficult datasets with higher noise ratios, we can achieve a significant improvement over the second-best model. Moreover, our proposed approach can easily be integrated into existing DNN methods to improve their robustness against label noise.

==> 02.related_work_old.tex <==
\section{Related Work}
%Label noise is ubiquitous and inevitable in the real world. Training DNNs with noisy labels can significantly deteriorate their performance.
There have been numerous approaches proposed to deal with noisy labels. These can generally be categorized into three types.
% correct the corrupted labels
The most straightforward way is to improve the quality of a dataset by cleaning up the corrupted samples. Samples that are identified as corrupted are either removed or corrected.
There have been multiple strategies proposed to identify the most likely corrupted samples, using directed graphical models~\cite{xiao2015learning},
conditional random fields~\cite{vahdat2017cdf},
knowledge graphs distilling knowledge from noisy data~\cite{li2017distill} and using a label cleaning network to achieve noise-robust classifications~\cite{veit2017learning}. 
However, auxiliary clean data are often required and not always obtainable.
%auxiliary clean data \textbf{are} often required which is not always obtainable.

% Modify the loss function
Another approach is to reformulate the loss function.
Patrini et al.~\shortcite{patrini2017forward} estimate the noise transition matrix and use it to adjust the loss function, while Ma et al.~\shortcite{ma2018d2l} correct the loss to avoid overfitting to noisy labels.
Some recent works attempt to exploit noise-tolerant losses. Theoretical studies by~\cite{ghosh2015making,ghosh2017robust} prove that the mean absolute error (MAE) is robust to label noise under certain assumptions. Inspired by Ghosh's work, other robust losses have been proposed~\cite{wang2019sl,zhang2018gce}.
%Wang et al.~\shortcite{wang2019sl} propose symmetric cross-entropy learning by balancing cross-entropy and a noise-tolerant reverse cross-entropy while \citet{zhang2018gce} propose a set of noise-tolerant loss functions that generalize both the categorical cross-entropy and MAE.
%These modified loss functions can often be directly incorporated into existing architectures without any prior knowledge of the true noise distribution.

Refinement of the training process has also been explored to deal with noisy labels.
Malach et al.~\shortcite{malach2017decoupling} design a novel framework that is similar to active learning, i.e., training on the samples in disagreement as estimated by two networks, and decouples ``when to update" with ``what to update". 
Ren et al.~\shortcite{ren2018reweight} use a meta-learning approach that assigns different weights to training samples based on their gradient directions, obtained by a meta gradient descent step on a clean validation dataset.
MentorNet~\cite{jiang2017mentornet} is proposed to supervise the training of a student network and make it focus on samples with a higher probability of being labeled correctly.
Following the same idea, Co-teaching~\cite{han2018coteach} trains a network with the most confident samples as output by a second network.
Apart from these, different augmentations to the network structure to model the label noise statistics have been proposed~\cite{goldberger2016layer,jindal2016dropout}.

In this work, we propose an approach in the context of refining the training process. The main innovation is the inclusion of $K$-fold cross-validation and the further use of an ensemble method to deal with noisy labels. 

